Measurement of the Relativistic Sunyaev-Zeldovich Corrections in RX J1347.5-1145

We present a measurement of the relativistic corrections to the thermal Sunyaev-Zel'dovich (SZ) effect spectrum, the rSZ effect, toward the massive galaxy cluster RX J1347.5-1145 by combining sub-mm images from Herschel-SPIRE with mm-wave Bolocam maps. Our analysis simultaneously models the SZ effect signal, the population of cosmic infrared background (CIB) galaxies, and galactic cirrus dust emission in a manner that fully accounts for their spatial and frequency-dependent correlations. Gravitational lensing of background galaxies by RX J1347.5-1145 is included in our methodology based on a mass model derived from HST observations. Utilizing a set of realistic mock observations, we employ a forward modelling approach that accounts for the non-Gaussian covariances between observed astrophysical components to determine the posterior distribution of SZ effect brightness values consistent with the observed data. We determine a maximum a posteriori (MAP) value of the average Comptonization parameter of the intra-cluster medium (ICM) within R$_{2500}$ to be $\langle y \rangle_{2500} = 1.56 \times 10^{-4}$, with corresponding 68~per cent credible interval $[1.42,1.63] \times 10^{-4}$, and a MAP ICM electron temperature of $\langle \textrm{T}_{\textrm{sz}} \rangle_{2500} = 22.4$~keV with 68~per cent credible interval spanning $[10.4,33.0]$~keV. This is in good agreement with the pressure-weighted temperature obtained from {\it Chandra} X-ray observations, $\langle \textrm{T}_{\textrm{x,pw}}\rangle_{2500} = 17.4 \pm 2.3$~keV. We aim to apply this methodology to comparable existing data for a sample of 39 galaxy clusters, with an estimated uncertainty on the ensemble mean $\langle \textrm{T}_{\textrm{sz}} \rangle_{2500}$ at the $\simeq 1$~keV level, sufficiently precise to probe ICM physics and to inform X-ray temperature calibration.

==> full_clus_sample.tex <==
% the complete cluster sample as of April 27, 2021
\begin{deluxetable*}{cccc}
\tablenum{2}
\tablecaption{Full Cluster Sample\label{tab:clus_sample}}
\tablewidth{0pt}
\tablehead{\colhead{Name} & \colhead{Redshift} & \colhead{RA} & \colhead{DEC}}
\startdata
    \cutinhead{Bolocam}
        Abell 209 & 0.21 & 01:31:53 & -13:36:48 \\
        Abell 370 & 0.38 & 02:39:53 & -01:34:38 \\
        Abell 383 & 0.19 & 02:48:03 & -03:31:46 \\
        Abell 611 & 0.29 & 08:00:56 & +36:03:25 \\
        Abell 697\tablenotemark{*} & 0.28 & 08:42:57 & +36:21:56 \\
        Abell 1689 & 0.18 & 13:11:29 & -01:20:27 \\
        Abell 1835\tablenotemark{*} & 0.25 & 14:01:01 & +02:52:40 \\
        Abell 2219 & 0.23 & 16:40:20 & +46:42:29 \\
        Abell 2744 & 0.31 & 00:14:15 & -30:23:31 \\
        Abell S1063 & 0.35 & 22:48:44 & -44:31:45 \\
        ZwCl0024.0 & 0.40 & 00:26:35 & +17:09:40 \\
        MACS J0025.4\tablenotemark{*} & 0.58 & 00:25:29 & -12:22:44 \\
        MACS J0717.5\tablenotemark{*} & 0.55 & 07:17:32 & +37:45:20 \\
        MACS J0744.9 & 0.70 & 07:44:52 & +39:27:27 \\
        MACS J1149.6 & 0.54 & 11:49:35 & +22:24:04 \\
        MACS J1423.8 & 0.54 & 14:23:47 & +24:04:43 \\
        MACS J0454.1\tablenotemark{*} & 0.54 & 04:54:11 & -03:00:50 \\
        MACS J2129.4\tablenotemark{*} & 0.59 & 21:29:26 & -07:41:28 \\
        MS 1054 & 0.83 & 10:56:58 & -03:37:33 \\
        MS 2137 & 0.31 & 21:40:15 & -23:39:40 \\
        RX J0152.7 & 0.83 & 01:52:41 & -13:58:06 \\
        RX J1347.5\tablenotemark{*} & 0.45 & 13:47:30 & -11:45:08 \\
    \cutinhead{ACT}
        Abell 68 & 0.255 & 00:36:59 & +09:08:30 \\
        Abell 368 & 0.220 & 02:37:25 & -26:30:02 \\
        Abell 521 & 0.253 & 04:54:10 & -10:15:11 \\
        Abell 868 & 0.153 & 09:42:57 & -08:38:51 \\
        Abell 2390 & 0.228 & 21:53:35 & +17:40:11 \\
        Abell 2537 & 0.295 & 23:08:16 & -02:10:44 \\
        Abell 2631 & 0.273 & 23:37:40 & +00:17:37 \\
        Abell 2667 & 0.230 & 23:51:47 & -26:00:18 \\
        Abell 2813 & 0.292 & 00:43:23 & -20:37:35 \\
        Abell 2895 & 0.227 & 01:18:05 & -27:00:13 \\
        Abell 3084 & 0.098 & 03:04:04 & -36:57:21 \\
        Abell 3088 & 0.253 & 03:07:01 & -28:40:30 \\
        Abell S0592 & 0.222 & 06:38:51 & -53:57:47 \\
        Abell S1077 & 0.312 & 22:58:52 & -34:46:55 \\
        Bullet & 0.296 & 06:58:29 & -55:57:10 \\
        RCS J2319.9 & 0.897 & 23:19:53 & +00:38:13 \\
        RCS J0224.5 & 0.773 & 02:24:30 & -00:02:00 \\
        RCS J2327 & 0.831 & 23:27:28 & -02:04:39 \\
\enddata
    \tablecomments{MACS J2129.4\tablenotemark{*} \victoria{this one is iffy and needs to be double checked, label from Adi says RX J2129.6}}
    \tablenotetext{*}{mass model completed using high quality HST data}
\end{deluxetable*}


==> mocks.tex <==
% This was for the original flux cutting procedure with just trimming based on brightest flux
Success rate using 21.7 mJy brightest source flux limit : 36.76\% 
Total failures : 172
Total Sims : 272

% new method values
The number of sims that only failed the maximum flux limit = 73
The number of sims that only failed the weighted sums = 22
The number of sims that failed only the minimum flux conf. limit = 1
The number of sims that failed the first two combined = 74
The number of sims that failed all three = 75
Success rate = 25\%

\subsection{Pipeline Flow}

\begin{enumerate}
    \item Read in real SPIRE data and define 3 band pixel scales, FWHM, and band centers
    \item Enter while loop condition which is only broken if PSW lensed flux checks have been passed, otherwise, new simulation is generated and lensed until condition is met
    \item Define CRVAL1 and CRVAL2 based on Bolocam template header info
    \item Read in catalog from either Conley or SIDES and mask all x,y positions outside of 0.25x0.25 degrees. This is then made into a lookup table which is sent to the lensing script
    \item Coordinates are in pixel space where (0,0) is in the center. The coordinates are adjusted so (0,0) sits within the middle of the real SPIRE field using CRPIX1/CRPIX2
    \item ASTROPY pixel to skycoord is used to convert the pixel coordinates to RA,DEC, this is then passed to FORMAT BETHERMIN.\\
    \textcolor{red}{Format Bethermin is heavily deprecated, since the new lensing code does not require any pre-processing beyond what has already been stated. The following is a relic of the usage necessary for LENSTOOL, but it is still used for testing and for creating output maps.}
        \begin{enumerate}
            \item The world coordinates above are converted back to pixel space using ASTROPY skycoord to pixel and the real SPIRE header for a given band
            \item For SIDES, we trim all of the sources that have a flux of zero
            \item Apply a flux cut mask
            \item Apply a redshift mask, sources with redshifts that are less than that of the cluster are removed and saved into a separate catalog
            \item Sources are sorted by brightness, where the maximum flux is first in the array. These sources are trimmed to the first 50,000 brightest sources if using LENSTOOL.
            \item Sources are sorted by redshift 
            \item Low redshift sources are added back into catalog
            \item The catalog is saved and sent to LENSTOOL
            \item The pre-lensed map is made using the model eval function from PCAT and returned to the main function
        \end{enumerate}
    \item The catalog is lensed using the Bolocam sized deflection field
    \item The output lensed map is created using POPMAP, where the lensed catalog is in units of arcseconds. The positions are divided by PSW pixel size and offset to be centered in the real SPIRE field using CRPIX1/CRPIX2. The pixels are converted to world coordinates again, and then converted back to the appropriate band pixel size using the SPIRE header and the previously mentioned ASTROPY packages. This catalog is given to the same PCAT model eval function.
    
    
    \item Here begins the flux trimming procedure, which is performed on only the PSW post lensed map
        \begin{enumerate}
            \item Sources from the post-lensed catalog are masked using the mu<1.5 ellipsoid condition.
            \item Enforce that the brightest source within this ellipse must be within the confusion noise limit of the brightest source from the real SPIRE PCAT catalog
            \item Mask all sources below the confusion noise limit, 11.6 mJy
            \item Compute SZ-template weighted sum for remaining sources
            \item Enforce condition that weighted sum must be within 2 sigma of the real SPIRE PCAT catalog weighted sum
            \item Any sims which don't meet every condition are remade from the top
        \end{enumerate}
        
        
    \item Trim every map object (signal, srcrm, xclean, sze, iris, planck, error, mask, noise, sig pre lens, sig post lens, exp) to 0.25x0.25 map size for a given band
    \item Generate noise map realization using the product of the error map and a random normalized gaussian distribution. The noise map is added to post-lensed map
    \item All map objects are added back into python dictionary and saved to a fits file. A history tag is added to the fits header stating the version of the sims and specific identifying characteristics, as well as the savefile date. 
\end{enumerate}

==> systematics.tex <==
% copied from https://docs.google.com/document/d/17c6uduz7UU_-KuCx3afo8VwqOU9ilVKa8W8oiH4yCTQ/edit?usp=sharing


